PingPong: Packet-Level Signatures for Smart Home Device Events

Smart home devices are vulnerable to passive inference attacks based on network traffic, even in the presence of encryption. In this paper, we present PINGPONG, a tool that can automatically extract packet-level signatures for device events (e.g., light bulb turning ON/OFF) from network traffic. We evaluated PINGPONG on popular smart home devices ranging from smart plugs and thermostats to cameras, voice-activated devices, and smart TVs. We were able to: (1) automatically extract previously unknown signatures that consist of simple sequences of packet lengths and directions; (2) use those signatures to detect the devices or specific events with an average recall of more than 97%; (3) show that the signatures are unique among hundreds of millions of packets of real world network traffic; (4) show that our methodology is also applicable to publicly available datasets; and (5) demonstrate its robustness in different settings: events triggered by local and remote smartphones, as well as by homeautomation systems.

==> Makefile <==
all:
	pdflatex main.tex
	bibtex main.aux
	pdflatex main.tex
	pdflatex main.tex
	@echo ================================================================
	pdflatex main.tex | grep -E 'arning|erfull'
	@echo ================================================================

spell:
	@for i in *.tex; \
	do if [ $$i != "paper.tex" ]; then aspell -c $$i -p ./spell.lst; fi;\
	done

clean:
	rm -f *.dvi *.log *.aux *.blg *.bbl *.out
	rm -f main.ps main.pdf
	rm -f main.synctex.gz




==> evaluation-old.tex <==
\section{Evaluation}
\label{sect:evaluation}
%In evaluating our methodology and \tool, we seek to answer the following
%questions.
%\myparagraph{Q1: How well does packet-level analysis generalize across different smart home devices?}
%That is, given our set of smart home devices, how many exhibit 
%packet-level signatures? %\label{enum:eval-q-generalize}
%\myparagraph{Q2: How well do our \tool parameters generalize across different smart home devices?}
%That is, given our set of smart home devices, how effective are \tool's parameters for training and 
%detection?
%\myparagraph{Q3: How well do the extracted packet-level signatures perform?} 
%That is, given an unseen network trace with a set of known 
%device events, how many of those events can \tool detect? %\label{enum:eval-q-accuracy}
%\myparagraph{Q4: How unique are the extracted packet-level signatures?} 
%If the signatures are not sufficiently unique, \tool will generate false positives. 
%\label{enum:eval-q-uniqueness}
%Sec.~\ref{sect:training-phase} addresses question \textbf{Q1},
%Sec.~\ref{sect:parameter-sensitivity} addresses question \textbf{Q2},  
%Sec.~\ref{sect:detection-phase} addresses question \textbf{Q3}, and 
%Sec.~\ref{sect:negative-control} addresses question \textbf{Q4}.


In this section, we present the evaluation of  \tool.
In  Section~\ref{sect:training-phase}, we show that  \tool was able to automatically extract strong event signatures for 12 out of 13 devices, as summarized in Table \ref{tab:summary-signatures}. Section~\ref{sect:parameter-sensitivity}  discusses the choice and sensitivity of parameters used to extract those signatures. % DBDSCAN, t
Section.~\ref{sect:detection-phase} uses the extracted signatures  to detect \events in a trace collected from a realistic experiment on our smart home testbed.
Section~\ref{sect:negative-control} presents the results of negative control experiments: it demonstrates the uniqueness of the \tool signatures in large  (\ie with tens of millions of packets), publicly available, packet traces from smart home and  office environments.

\begin{table}[t!]
  \centering
  \begin{center}
  { %\footnotesize
  \small
  \begin{tabular}{| p{35mm} | c | c | c |}
    \hline
    	\textbf{Device} & \textbf{Device-} & \textbf{Phone-} & \textbf{Phone-}\\
    	& \textbf{Cloud} & \textbf{Cloud} & \textbf{Device}\\
    \hline
    	\amazonplug & \cellcolor{green} \checkmark & $\times$ & $\times$ \\
    \hline
    	\wemoplug & $\times$ & $\times$ & \cellcolor{green} \checkmark\\
    \hline
    	\wemoinsightplug & $\times$ & $\times$ & \cellcolor{green} \checkmark\\
    \hline
    	\sengledbulb & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & $\times$ \\
    \hline
    	\huebulb & $\times$ & $\times$ & \cellcolor{green} \checkmark\\
    \hline
        \nestthermostat & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \ecobeethermostat & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \rachiosprinkler & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \arlocamera & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \roombarobot & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \ringalarm & \cellcolor{green} \checkmark & $\times$ & $\times$\\
    \hline
        \tplinkplug & \cellcolor{green} \checkmark & $\times$ & \cellcolor{green} \checkmark\\
    \hline
        \dlinkplug & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \dlinksiren & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
    	\tplinkbulb & $\times$ & $\times$ & \cellcolor{green} \checkmark\\
    \hline
        \smartthingsplug & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \blossomsprinkler & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & $\times$\\
    \hline
        \kwiksetdoorlock & $\times$ & \cellcolor{green} \checkmark & $\times$\\
    %\hline
    %	\lifxbulb & $\times$ & $\times$ & $\times$\\
    %\hline
    %	\multicolumn{2}{| c |}{\cellcolor{green} \checkmark = signature found} & 
    %	\multicolumn{2}{| c |}{$\times$ = signature not found}\\
    \hline
  \end{tabular}
  }
  \end{center}
  \caption{Summary of Signatures (\checkmark = signature extracted; $\times$ = signature not found).
  	\label{tab:summary-signatures}}
\end{table}
  	
\begin{table*}[t!]
  \centering
  \begin{center}
  { %\footnotesize
  \small
  \begin{tabular}{| p{15mm} | p{18mm} | c | c | c | c | c | c | c |}
    \hline
        & & & & & \multicolumn{4}{| c |}{\textbf{Matching}}\\
        \textbf{Device} & \textbf{Feature} & \textbf{Signature} & \textbf{Comm.} & \textbf{Duration (ms)} & \multicolumn{4}{| c |}{\textbf{(Per 100 Events)}}\\
    \cline{6-9}
        & & & & \textbf{Min./Avg./Max.} & \textbf{WAN} & \textbf{Fal.} & \textbf{Wi-Fi} & \textbf{Fal.}\\
        & & & & & \textbf{Snif.} & \textbf{Pos.} & \textbf{Snif.} & \textbf{Pos.}\\
	\hline
        Amazon & ON & \textbf{S1:} S-[443-445] & \devicecloudcomm & 1,232 / 2,465 / 4,537 & 98 & 0 & 99 & 0\\
        plug & & \textbf{S2:} C-1099 S-235 & & & & & &\\
	\cline{2-3}
        & OFF & \textbf{S1:} S-[444-446] & & & & & &\\
        & & \textbf{S2:} C-1179 S-235 & & & & & &\\
        & & \textbf{S3:} C-1514 C-103 S-235 & & & & & &\\
	\hline
        WeMo plug & ON/OFF & \textbf{S1:} PH-259 PH-475 D-246 & \phonedevicecomm & 33 / 42 / 134 & N/A & N/A & 100 & 0\\
	\hline
        WeMo & ON/OFF & \textbf{S1:} PH-259 PH-475 D-246 & \phonedevicecomm & 32 / 39 / 97 & N/A & N/A & 99 & 0\\
        Insight plug & & & & & & & &\\
	\hline
        Sengled & ON & \textbf{S1:} S-[217-218] C-[209-210] & \devicecloudcomm & 4,304 / 6,238 / 8,145 & 97 & 0 & N/A & N/A\\
        light bulb & & \textbf{S2:} C-430 & & & & & &\\
        & & \textbf{S3:} C-466 & & & & & &\\
	\cline{2-3}
        & OFF & \textbf{S1:} S-[217-218] C-[209-210] & & & & & &\\
        & & \textbf{S2:} C-430 & & & & & &\\
        & & \textbf{S3:} C-465 & & & & & &\\
	\cline{2-9}
        & ON & \textbf{S1:} C-211 S-1063 & \phonecloudcomm & 4,375 / 6,356 / 9,132 & 93 & 0 & 97 & 0\\
        & & \textbf{S2:} S-1277 & & & & & &\\
	\cline{2-3}
        & OFF & \textbf{S1:} C-211 S-1063 S-1276 & & & & & &\\
	\cline{2-9}
        & Intensity & \textbf{S1:} S-[216-220] & \devicecloudcomm & 16 / 74 / 824 & 99 & 2 & N/A & N/A\\
        & & C-[208-210] & & & & & &\\
	\cline{2-9}
        & Intensity & \textbf{S1:} C-[215-217] & \phonecloudcomm & 3,916 / 5,573 / 7,171 & 99 & 0 & 99 & 0\\
        & & S-[1275-1277] & & & & & &\\
	\hline
        Hue light & ON & \textbf{S1:} PH-229 D-569 & \phonedevicecomm & 12 / 14 / 25 & N/A & N/A & N/A & N/A\\
	\cline{2-3}
        bulb & OFF & \textbf{S1:} PH-230 D-570 & & & & & &\\
    \hline
    	Nest & Fan ON & \textbf{S1:} C-[891-894] S-[830-834] & \phonecloudcomm & 91 / 111 / 1,072 & 93 & 0 & 92 & 1\\
    \cline{2-3}
    	thermostat & Fan OFF & \textbf{S1:} C-[858-860] S-[829-834] & & & & & &\\
    	%& & & & & & & &\\
   	\hline
        Ecobee & HVAC Auto & \textbf{S1:} S-1300 C-640 & \phonecloudcomm & 121 / 229 / 667 & 100 & 0 & 99 & 0\\
	\cline{2-3}
        thermostat & HVAC OFF & \textbf{S1:} C-1299 C-640 & & & & & &\\
	\cline{2-9}
        & Fan ON & \textbf{S1:} S-1387 C-640 & \phonecloudcomm & 117 / 232 / 1,776 & 100 & 0 & 100 & 0\\
	\cline{2-3}
        & Fan Auto & \textbf{S1:} C-1389 C-640 & & & & & &\\
	\hline
        Rachio & Quick Run & \textbf{S1:} S-267 C-155 & \devicecloudcomm & 1,972 / 2,180 / 2,450 & 100 & 0 & 100 & 0\\
	\cline{2-3}
        sprinkler & Stop & \textbf{S1:} C-496 C-155 C-395 & & & & & &\\
	\cline{2-9}
        & Standby/ & \textbf{S1:} S-299 C-155 C-395 & \devicecloudcomm & 276 / 690 / 2,538 & 100 & 0 & 100 & 0\\
        & Active & & & & & & &\\
    \hline
        Arlo & Stream ON & \textbf{S1:} C-[338-339] S-[326-329] & \phonecloudcomm & 46 / 78 / 194 & 99 & 2 & 98 & 3\\
        camera & & C-[364-365] S-[1061-1070] & & & & & &\\
        & & \textbf{S2:} C-[271-273] S-[499-505] & & & & & &\\
        %& & & & & & & &\\
	\cline{2-3}
        & Stream OFF & \textbf{S1:} C-[445-449] S-442 & & & & & &\\
        %& & & & & & & &\\
	\hline
        Roomba & Clean & \textbf{S1:} S-[1014-1015] C-105 & \phonecloudcomm & 123 / 2,038 / 5,418 & 91 & 0 & 91 & 0\\
        robot & & S-432 C105 & & & & & &\\
	\cline{2-3}
        & Back-to- & \textbf{S1:} S-440 C-105 & & & & & &\\
        & station & S-[1018-1024] C-105 & & & & & &\\
	\hline
        Ring & Arm & \textbf{S1:} S-99 S-254 C-99 & \devicecloudcomm & 275 / 410 / 605 & 98 & 0 & 98 & 0\\
        alarm & & S-[181-183] C-99 & & & & & &\\
	\cline{2-3}
        & Disarm & \textbf{S1:} S-99 S-255 C-99 & & & & & &\\
        & & S-[181-183] C-99 & & & & & &\\
	\hline
        TP-Link & ON & \textbf{S1:} C-556 S-1293 & \devicecloudcomm & 75 / 85 / 204 & 99 & 0 & 99 & 0\\
    \cline{2-3}
        plug & OFF & \textbf{S1:} C-557 S-[1294-1295] & & & & & &\\
        %& & & & & & & &\\
    \cline{2-9}
        & ON/OFF & \textbf{S1:} PH-112 D-115 & \phonedevicecomm & 2 / 4 / 39 & N/A & N/A & N/A & N/A\\
        %& & & & & & & &\\
	\hline
        D-Link & ON/OFF & \textbf{S1:} S-91 S-1227 C-784 & \devicecloudcomm & 4 / 1,194 / 8,060 & 95 & 0 & 95 & 0\\
        plug & & \textbf{S2:} C-1052 S-647 & & & & & &\\
    \cline{2-9}
    	& ON & \textbf{S1:} C-[1109-1123] S-613 & \phonecloudcomm & 35 / 41 / 176 & 98 & 0 & 98 & 0\\
    \cline{2-3}
        & OFF & \textbf{S1:} C-[1110-1124] S-613 & & & & & &\\
    \hline
        D-Link & ON & \textbf{S1:} C-1076 S-593 & \phonecloudcomm & 36 / 37 / 65 & 100 & 0 & 98 & 0\\
	\cline{2-3}
        siren & OFF & \textbf{S1:} C-1023 S-613 & & & & & &\\
	\hline
        TP-Link & ON & \textbf{S1:} PH-198 D-227 & \phonedevicecomm & 8 / 77 / 148 & N/A & N/A & 100 & 4\\
	\cline{2-3}
        light bulb & OFF & \textbf{S1:} PH-198 D-244 & & & & & &\\
    \cline{2-9}
        & Intensity & \textbf{S1:} PH-[240-242] D-[287-289] & \phonedevicecomm & 7 / 84 / 212 & N/A & N/A & 100 & 0\\
    \cline{2-9}
        & Color & \textbf{S1:} PH-317 D-287 & \phonedevicecomm & 6 / 89 / 174 & N/A & N/A & 100 & 0\\
    \hline
  \end{tabular}
  }
  \end{center}
  %\caption{Smart home devices found to exhibit \phonecloudcomm, \devicecloudcomm, and \phonedevicecomm signatures 
  %	(prefix PH indicates Phone-to-device direction and prefix D indicates Device-to-phone direction;
  %	the duration of each signature is measured from the first packet of 
  %	the first sequence S1 to the last packet of the last sequence Sn).
  %	\label{tab:wan-signatures}}
\end{table*}

\begin{table*}[t!]
  \centering
  \begin{center}
  { %\footnotesize
  \small
  \begin{tabular}{| p{15mm} | p{18mm} | c | c | c | c | c | c | c |}
    \hline
        & & & & & \multicolumn{4}{| c |}{\textbf{Matching}}\\
        \textbf{Device} & \textbf{Feature} & \textbf{Signature} & \textbf{Comm.} & \textbf{Duration (ms)} & \multicolumn{4}{| c |}{\textbf{(Per 100 Events)}}\\
    \cline{6-9}
        & & & & \textbf{Min./Avg./Max.} & \textbf{WAN} & \textbf{Fal.} & \textbf{Wi-Fi} & \textbf{Fal.}\\
        & & & & & \textbf{Snif.} & \textbf{Pos.} & \textbf{Snif.} & \textbf{Pos.}\\
    \hline
        Smart- & ON & \textbf{S1:} C-699 S-511 & \phonecloudcomm & 335 / 537 / 2,223 & 92 & 0 & 92 & 0\\
        Things & & \textbf{S2:} S-777 C-136 & & & & & &\\
	\cline{2-3}
        plug & OFF & \textbf{S1:} C-700 S-511 & & & & & &\\
        & & \textbf{S2:} S-780 C-136 & & & & & &\\
	\hline
        Blossom & Quick Run & \textbf{S1:} C-326 & \devicecloudcomm & 701 / 3,470 / 8,431 & 96 & 0 & 96 & 0\\
        sprinkler & & \textbf{S2:} C-177 S-505 & & & & & &\\
	\cline{2-3}
        & Stop & \textbf{S1:} C-326 & & & & & &\\
        & & \textbf{S2:} C-177 S-458 & & & & & &\\
        & & \textbf{S3:} C-238 C-56 S-388 & & & & & &\\
    \cline{2-9}
        & Quick Run & \textbf{S1:} C-649 S-459 C-574 S-507 & \phonecloudcomm & 70 / 956 / 3,337 & 93 & 0 & 93 & 0\\
        & & \textbf{S2:} S-[135-139] & & & & & &\\
	\cline{2-3}
        & Stop & \textbf{S1:} C-617 S-431 & & & & & &\\
    \cline{2-9}
        & Hibernate & \textbf{S1:} C-621 S-493 & \phonecloudcomm & 121 / 494 / 1,798 & 95 & 0 & 93 & 0\\
	\cline{2-3}
        & Active & \textbf{S1:} C-622 S-494 & & & & & &\\
        & & \textbf{S2:} S-599 C-566 S-554 C-566 & & & & & &\\
    \hline
        Kwikset & Lock & \textbf{S1:} C-699 S-511 & \phonecloudcomm & 173 / 395 / 2,874 & 100 & 0 & 100 & 0\\
        door & & \textbf{S2:} S-639 C-136 & & & & & &\\
	\cline{2-3}
        lock & Unlock & \textbf{S1:} C-701 S-511 & & & & & &\\
        & & \textbf{S2:} S-647 C-136 & & & & & &\\
    \hline
  \end{tabular}
  }
  \end{center}
  \caption{Smart home devices found to exhibit \phonecloudcomm, \devicecloudcomm, and \phonedevicecomm signatures 
  	(prefix PH indicates Phone-to-device direction and prefix D indicates Device-to-phone direction;
  	the duration of each signature is measured from the first packet of 
  	the first sequence S1 to the last packet of the last sequence Sn).
  	\label{tab:wan-signatures}}
\end{table*}

%\begin{table*}[t!]
%  \centering
%  \begin{center}
%  { \footnotesize
%  \begin{tabular}{| p{22mm} | c | c | c | c | c | c |}
%    \hline
%        \textbf{Device} & \multicolumn{2}{| c |}{\textbf{Signature (Phone - Device)}} & \textbf{Duration (ms)} & \textbf{Validation} & \textbf{Wi-Fi Sniffer Matching} & \textbf{False}\\
%    \cline{2-3}
%    	& \textbf{ON} & \textbf{OFF} & \textbf{Min./Avg./Max.} & \textbf{(Result per 100 events)} & \textbf{(Result per 100 events)} & \textbf{Positive}\\
%    \hline
%        \tplinkplug* & \multicolumn{2}{| c |}{S1: PH-112 D-115} & 2 / 4 / 39  & 100 & N/A & N/A\\
%    \hline
%        \tplinkbulb & S1: PH-198 D-227 & S1: PH-198 D-244 & 8 / 77 / 148 & 100 & 100 & 0\\
%    \hline
%        \huebulb & S1: PH-229 D-569 & S1: PH-230 D-570 & 12 / 14 / 25 & 100 & N/A & N/A\\
%    \hline
%        \wemoplug & \multicolumn{2}{| c |}{S1: PH-259 PH-475 D-246} & 33 / 42 / 134 & 100 & 100 & 0\\
%    \hline
%        \wemoinsightplug & \multicolumn{2}{| c |}{S1: PH-259 PH-475 D-246} & 32 / 39 / 97 & 100 & 100 & 0\\
%    \hline
%  \end{tabular}
%  }
%  \end{center}
%  \caption{Smart home devices found to exhibit \phonedevicecomm signatures 
%  	(note that the TP-Link plug has both \devicecloudcomm and \phonedevicecomm signatures*;
%  	prefix PH indicates Phone-to-device direction and prefix D indicates Device-to-phone direction;
%  	the duration of each signature is measured from the first packet of 
%  	the first sequence S1 to the last packet of the last sequence Sn).
%  	\label{tab:lan-signatures}}
%\end{table*}

\subsection{Extracting Signatures from 13 Smart Home Devices}
\label{sect:training-phase}
\myparagraph{Training Dataset.} In order to evaluate the generalizability of packet-level analysis, we first
used \tool to automate the collection of training sets (see 
Sec.~\ref{sect:data-collection}) for 13 different smart home devices, 
including smart plugs, light bulbs, a door lock, a thermostat, a siren, a
sprinkler, and a surveillance camera (see Table~\ref{tab:smarthome-devices}). 
%Ten of these devices connect directly to
%the home router using Wi-Fi, while the remaining three devices are Zigbee-based
%devices that connect indirectly through a Zigbee hub (\ie the SmartThings Hub
%or the Philips Hue Hub) that is then connected to the router using an Ethernet
%cable.
Training sets were collected for every device under test, individually 
without any Background Traffic (see Fig.~\ref{fig:combined-setup}).
The automation script generated a total of 100 events 
for the device (\eg 50 ON and 50 OFF events for a smart plug, and 
50 LOCK and 50 UNLOCK events for a door lock).

\myparagraph{Results Summary.} For each training set, we next used \tool to extract packet-level signatures 
(see Sec.~\ref{sect:system-training}) for each event type 
of the respective device. 
In summary, \tool extracted signatures from 12 out of 13 devices;
see Table~\ref{tab:summary-signatures}.
\tool found packet-level signatures
that are observable in the device's \phonecloudcomm and \devicecloudcomm communications.
\tool also found packet-level signatures that are only observable in the device's
\phonedevicecomm communication. 
%We next elaborate on the discovered signatures.
% and save them into signature files based on event types, 
%\eg one ON event signature file and one OFF event signature file for a 
%smart plug (see Sec.~\ref{sect:system-training}).

%\begin{table*}[t!]
%  \centering
%  \begin{center}
%  { \footnotesize
%  \begin{tabular}{| p{22mm} | c | c | c | c | c | c | c | c | c |}
%    \hline
%        \textbf{Device} & \multicolumn{2}{| c |}{\textbf{Validation}} & \multicolumn{3}{| c |}{\textbf{WAN Sniffer Matching}} &  \multicolumn{3}{| c |}{\textbf{Wi-Fi Sniffer Matching}} \\
%    \cline{4-9}
%        & \multicolumn{2}{| c |}{\textbf{(Result per 100 events)}} & \multicolumn{2}{| c |}{\textbf{Result per 100 events}} & \textbf{False} & \multicolumn{2}{| c |}{\textbf{Result per 100 events}} & \textbf{False}\\
%    \cline{2-5}
%    \cline{7-8}
%    	& \textbf{Device-Cloud} & \textbf{Phone-Cloud} & \textbf{Device-Cloud} & \textbf{Phone-Cloud} & \textbf{Positive} & \textbf{Device-Cloud} & \textbf{Phone-Cloud} & \textbf{Positive}\\
%    \hline
%        \dlinkplug & 97 & 100 & 95 & 98 & 0 & 95 & 98 & 0\\
%    \hline
%        \tplinkplug & 100 & N/A & 99 & N/A & 0 & 99 & N/A & 0\\
%    \hline
%        \dlinksiren & N/A & 100 & N/A & 100 & 0 & N/A & 100 & 0\\
%    \hline
%        \smartthingsplug & N/A & 98 & N/A & 92 & 0 & N/A & 97 & 0\\
%    \hline
%        \kwiksetdoorlock & N/A & 98 & N/A & 100 & 0 & N/A & 100 & 0\\
%    \hline
%        \arlocamera & N/A & 99 & N/A & 97* & 2 & N/A & 97* & 2\\
%    \hline
%        \nestthermostat & N/A & 100 & N/A & 93 & 0 & N/A & 93 & 3\\
%    \hline
%        \blossomsprinkler & 98 & 98 & 96 & 93 & 0 & 96 & 93 & 0\\
%    \hline
%  \end{tabular}
%  }
%  \end{center}
%  \caption{Signature validation and matching results for devices with \phonecloudcomm and \devicecloudcomm signatures
%  	(97 events were detected for Arlo camera after using only set S1
%  	for the ON-signature*; Wi-Fi Sniffer Matching for TP-Link plug combines \devicecloudcomm and \phonedevicecomm signatures).
%  	\label{tab:wan-signatures-accuracy}}
%\end{table*}

%\subsubsection{WAN Signatures}
\myparagraph{\phonecloudcomm \& \devicecloudcomm Signatures.}
%Our threat model focuses on adversaries that observe traffic at or
%upstream from the WAN interface of the router (see Sec.~\ref{sect:threat-model}).
8 out of 13 devices have signatures that are observable in the
device's \phonecloudcomm or \devicecloudcomm communication, or both.
%This traffic stems from communication between the
%device itself and some Internet host, or communication between the
%controlling smartphone and some Internet host. 
Although the traffic is typically encrypted
using TLSv1.2,  the device event
still manifests itself in the form of a packet-level signature.
Table~\ref{tab:wan-signatures} summarizes the signatures that \tool was able to identify.
%, while the self-test results for signature validation (\ie matching the signature against the training set used to generate it; see Sec.~\ref{sect:system-training}) are summarized in Table~\ref{tab:wan-signatures-accuracy}. \todo{What are selt-tests  Is that standard terminology?}
In Table~\ref{tab:wan-signatures}, each line in a signature cell represents 
a packet sequence set, and the vertical positioning of these lines reflects
the ordering of the packet sequence sets in the signature; see 
Sec.~\ref{sect:system-training} for the notation definition. 
%\todo{Convoluted to talk about vertical positioning. Can we add line numbers to table?}
%We next elaborate on a couple of devices' WAN signatures, while we let
%Table~\ref{tab:wan-signatures} speak on behalf of the rest of the devices.

%All of these signatures were found in TLSv1.2 encrypted communication.
%Finally, all of these devices use TLSv1.2 encryption for their communication with
%cloud servers, but \tool does not perform deep packet inspection on the encrypted payload
%(see Sec.~\ref{sect:threat-model}).

\mysubparagraph{\dlinkplug.}
This device exhibits signatures in the \devicecloudcomm
\emph{and} \phonecloudcomm communications.
The signature present in the device's own communication consists
of two packet sequence sets, each of which have only one member.
This means that there was no variation in the packet length sequences
observed during training. That is, for all 100 events, the exact same
pattern occurs after every ON/OFF event: the packet sequence \code{S1: C-91 S-1227 C-784}
appears followed by the packet sequence \code{S2: C-1052 S-647}.
%What this means is that the incredibly deterministic: both of its two packet sequence sets only have one member
%each, meaning that the packet sequences (\ie \code{C-91 S-1227 C-784} and
%\code{C-1052 S-647}) look \emph{exactly} the same across all 100 events.
However, this also means that the extracted signature does not
differentiate ON from OFF as it is the same for both. 
The signatures present in the smartphone's communication are shorter and
less deterministic, but are able to differentiate between ON and OFF events.
For ON events, the signature's first packet's length is in the set
$\left\{1109, 1111, 1113, 1115, 1117, 1119, 1121, 1123\right\}$, whereas for 
OFF events, the signature's first packet's length is in the set
$\left\{1110, 1112, 1114, 1116, 1118, 1120, 1122, 1124\right\}$. Notice that while the two
signatures overlap in terms of their ranges, the length of the first packet in the
ON signature is always even, whereas it is odd in the case of the OFF signature.
%The self-test for the device-side signatures managed to detect 97 out of 100 
%events because the signatures were only partially present in 3 events.\todo{Need Rahmadi to elaborate on this self-test thing}

\mysubparagraph{\tplinkplug.}
This device exhibits signatures in the \devicecloudcomm communication, which are completely deterministic---there is only \emph{one} 
packet sequence in each packet sequence set. They differentiate 
ON vs OFF events---each event has a single, unique packet sequence associated with it.
%there is one packet sequence set per event type, and the single packet sequence in each packet sequence set is different from the single packet sequence in the other packet sequence set). 

\mysubparagraph{\dlinksiren.}  This device exhibits both ON and OFF
signatures in the \phonecloudcomm communication.  These signatures
have no variation in the packet sequences.
%These signatures are unique and they differentiate ON and OFF events;
%each signature has only one sequence per cluster.

\mysubparagraph{\smartthingsplug.}
This device exhibits both an ON signature and an OFF signature in the
\phonecloudcomm communication.
Both signatures are comprised of two packet sequence sets,
each with  only one packet 
pair.\footnote{Please note that while our preliminary observation presented in 
Sec.~\ref{sect:network-behavior} suggested that the members of the 
second set of packet sequences \code{S2} of both the ON and OFF signature should
be packet sequences of four packets, those longer sequences were truncated to
just two packets by the clustering process in the system training phase because
the frequency of the first packet pair of the longer packet sequence was below
the \code{minPts} threshold (see Sec.~\ref{sect:system-training}).}
There was no variation in the packet lengths observed during 
training.

\mysubparagraph{\kwiksetdoorlock.}
This exhibits signatures in the \phonecloudcomm communication, which
are distinct for LOCK and UNLOCK events.
Each signature is comprised of two packet sequence sets, each of which has 
only one member.
There was no variation in the packet lengths observed during 
training.
%This device has signatures only for smartphone side.
%These signatures are unique and they differentiate lock and unlock events;
%each signature has two clusters (each has one sequence variation).
%The self-test for the signatures managed to detect 98 of 100 events because 
%the signatures were only partially present in 3 events.

%The self-test for the signatures managed to detect 98 of 100 events because 
%the signatures were only partially present in 3 events.
%The self-test for the signatures managed to detect 99 of 100 events because 
%the ON signature was not present in 1 ON event.

\mysubparagraph{\arlocamera.}
This device exhibits signatures in the \phonecloudcomm communication.
The signatures are different for ON and OFF events and
the ON signature has some variation in its last packet's length. 
This signature is one of the 
longest signatures as it comprised of a packet sequence set of four packets, 
followed by a packet sequence set of two packets.
%This device has signatures only for smartphone side.
%These signatures are unique and they differentiate ON and OFF events.
%The ON event signature has two clusters with sequences of 4 and 2 packets.
%The OFF event signature has two clusters with sequences of 2 packets.
Details about the \arlocamera signature are depicted on Fig. \ref{fig:clustering-signature}(b) and have been extensively discussed there.

\mysubparagraph{\nestthermostat.}
This device exhibits signatures in the \phonecloudcomm communication.
The signatures are different for ON and OFF events.
Both signatures have slight variations: there are a variety of packet 
sequences in each set of packet sequences.
%This device has signatures only for smartphone side.
%These signatures are unique and they differentiate ON and OFF events for 
%the thermostat's fan control.

\mysubparagraph{\blossomsprinkler.}
This device exhibits signatures in both the \devicecloudcomm and \phonecloudcomm communications, which 
are different for ON and OFF events.
For the signatures present in the \devicecloudcomm communication, the ON  signature consists
of two packet sequence sets, while the OFF-event signature consists of three packet sequence sets.
For the signatures present in the \phonecloudcomm communication, the ON signature consists
of three packet sequence sets, while the OFF-event signature consists of one packet sequence set.
%Differentiation between ON and OFF is possible for both the device's and smartphone's communications 
%since the signatures are different for ON and OFF events.

%\begin{table*}[t!]
%  \centering
%  \begin{center}
%  { \footnotesize
%  \begin{tabular}{| p{22mm} | c | c | c | c | c | c |}
%    \hline
%        \textbf{Device} & \multicolumn{2}{| c |}{\textbf{Signature (Phone - Device)}} & \textbf{Duration (ms)} & \textbf{Validation} & \textbf{Wi-Fi Sniffer Matching} & \textbf{False}\\
%    \cline{2-3}
%    	& \textbf{ON} & \textbf{OFF} & \textbf{Min./Avg./Max.} & \textbf{(Result per 100 events)} & \textbf{(Result per 100 events)} & \textbf{Positive}\\
%    \hline
%        \tplinkplug* & \multicolumn{2}{| c |}{S1: PH-112 D-115} & 2 / 4 / 39  & 100 & N/A & N/A\\
%    \hline
%        \tplinkbulb & S1: PH-198 D-227 & S1: PH-198 D-244 & 8 / 77 / 148 & 100 & 100 & 0\\
%    \hline
%        \huebulb & S1: PH-229 D-569 & S1: PH-230 D-570 & 12 / 14 / 25 & 100 & N/A & N/A\\
%    \hline
%        \wemoplug & \multicolumn{2}{| c |}{S1: PH-259 PH-475 D-246} & 33 / 42 / 134 & 100 & 100 & 0\\
%    \hline
%        \wemoinsightplug & \multicolumn{2}{| c |}{S1: PH-259 PH-475 D-246} & 32 / 39 / 97 & 100 & 100 & 0\\
%    \hline
%  \end{tabular}
%  }
%  \end{center}
%  \caption{Smart home devices found to exhibit \phonedevicecomm signatures 
%  	(note that the TP-Link plug has both \devicecloudcomm and \phonedevicecomm signatures*;
%  	prefix PH indicates Phone-to-device direction and prefix D indicates Device-to-phone direction;
%  	the duration of each signature is measured from the first packet of 
%  	the first sequence S1 to the last packet of the last sequence Sn).
%  	\label{tab:lan-signatures}}
%\end{table*}

\myparagraph{\phonedevicecomm Signatures.}
%\subsubsection{LAN Signatures}
%Although our threat model (see Sec.~\ref{sect:threat-model}) is 
%concerned with WAN signatures, it turned out that \tool also 
%managed to extract packet-level signatures from the local communication
%between the smartphone and device (\ie referred to as LAN signatures).
\tool also extracted signatures from the \phonedevicecomm communication
for 5 out of 13 devices (see Table~\ref{tab:lan-signatures}).
%The signatures are summarized in Table~\ref{tab:lan-signatures}.
%The prefixes \code{PH} and \code{D} indicate the directions of the 
%packets---\code{PH} for \emph{Phone-to-device} and \code{D} for 
%\emph{Device-to-phone}, while the numbers indicate the lengths of 
%the packets as usual.
%\todo{We really overuse P...}
The signatures of all 5 devices are completely deterministic---no variations 
in packet lengths, but differentiation between ON 
and OFF is only possible for two devices (\ie \tplinkplug and \huebulb).
%In conclusion, a local adversary may also perform a packet-level 
%analysis based attack, but this is of lesser concern since (1) it 
%assumes a more privileged adversary, (2) event-specific signatures 
%are less prevalent, and (3) the communication between the smart 
%home device and the smartphone is generally unencrypted, which enables 
%more severe attacks that rely on deep packet inspection.

%\begin{table}[t!]
%  \centering
%  \begin{center}
%  { \footnotesize
%  \begin{tabular}{| p{45mm} | r | r | c | c |}
%    \hline
%        \textbf{Device} & \textbf{D} & \textbf{$\epsilon$} & \textbf{$\mathtt{minPts}$} & \textbf{Range}\\
%    \hline
%		\multicolumn{5}{| c |}{\textbf{Devices with WAN signatures}}\\
%    \hline
%        D-Link DCH-S220 & 1 & 1 & 48 & 48-49\\
%    \hline
%    	Kwikset SmartCode 910 & 1 & 1 & 48 & 48-50\\
%    \hline
%    	Arlo Q & 10 & 5 & 49 & 49-50\\
%    \hline
%    	Nest T3007ES & 5 & 3 & 50 & 50\\
%    \hline
%    	Blossom 7 Smart Watering Controller & 1 & 1 & 48 & 48-50\\
%    \hline
%		\multicolumn{5}{| c |}{\textbf{Devices with LAN signatures}}\\
%    \hline
%        TP-Link HS-100 & 1 & 1 & 50 & 50\\
%    \hline
%        TP-Link LB-130 & 1 & 1 & 50 & 50\\
%    \hline
%        Philips Hue white & 1 & 1 & 50 & 50\\
%    \hline
%        Belkin WeMo & 1 & 1 & 50 & 50\\
%    \hline
%        Belkin WeMo Insight & 1 & 1 & 50 & 50\\
%    \hline
%  \end{tabular}
%  }
%  \end{center}
%  \caption{DBSCAN parameters evaluation for devices under test
%  		(\textbf{D}=diameter; see Table~\ref{tab:dbscan-parameters}
%  		for TP-Link, D-Link, and Samsung SmartThings smart plugs).\label{tab:dbscan-parameters-all}}
%\end{table}

%\subsubsection{False Positives and Invalid Signatures.}
\myparagraph{Signature Validity.}
When \tool has a candidate signature, it performs
\emph{signature validation} before it finalizes the candidate as a signature;
see Sec.~\ref{sect:system-training} for details.
\footnote{
Recall that signature validation filters the
signature candidates that are not sufficiently unique to represent an event.
This can for example be the case when the signature is generated from 
traffic that happens to be present in the time window \timewindow, 
but which also occurs during the subsequent idle period (see Sec.~\ref{sect:system-training}).
We saw a manifestation of this for one device, namely the \lifxbulb.
We then drop such the signature candidates.
}
The validation results  are reported in a column in 
Tables~\ref{tab:wan-signatures} and \ref{tab:lan-signatures}.
In some cases, the validation does not capture all 100 events.
Manual inspection revealed that in these few cases, the signatures were 
only partially present or they are present with more variations, \eg
\code{S2: S-777 C-136} for the SmartThings plug might become
\code{S2: S-612 C-136} in some occasions.
%\todo{Partial presence part might generate 
%questions/perhaps not clear to reader. Rahmadi to elaborate?}
%Indeed, the \code{minPts} threshold used in the clustering process 
%(see Sec.~\ref{sect:system-training}) allows for a small deviation from 
%the number of events for exactly this purpose (\ie to enable recognition 
%of signatures that have a few outliers).
%As a consequence, whenever a signature with one or more packet 
%sequence sets with $<n$ members, where $n$ is the 
%number events performed during training, the number of events 
%that can be detected during validation is upper bounded by the number of 
%elements in the smallest packet sequence set plus the number of false 
%positives, if any.



\subsection{Parameters Selection and Sensitivity}
\label{sect:parameter-sensitivity}
\myparagraph{Clustering Parameters.}
We empirically examined a range of values for the parameters
of the DBSCAN algorithm. % to understand the sensitivity out our approach to the parameters.
We tried all combinations 
of $\epsilon \in \left\{ 1, 2,..., 10 \right\}$ and
$\mathtt{minPts} \in \left\{ 30, 31, ..., 50 \right\}$.
We only briefly summarize the results, due to lack of space.
For those devices that exhibit no variation in their signature related 
packet lengths, \eg the \tplinkplug, the output of the clustering remains stable
for all values of $\epsilon$ and $\mathtt{minPts} < 50$. 
%as the points lie on top of one another.
For such devices, keeping $\epsilon$ at a minimum and $\mathtt{minPts}$ close 
to the number of events $n$ reduces the number of noise points that become part of the resulting clusters.
However, our experiments  showed that applying such a strict
bound to devices with more variation in their packet lengths
(\eg the \dlinkplug), results in  losing
clusters that contain packet pairs related to \events. For the \dlinkplug, this happens if 
$\epsilon < 7$ and $\mathtt{minPts} > 47$. This therefore validates our choice of $\epsilon=10$ and $\mathtt{minPts}=45$
(\ie $\mathtt{minPts}=\lfloor n-0.1n \rfloor$ with $n$ = number of expected events)
as the default starting point when analyzing new devices. 
%\todo{Wrote section in the blind as I did not have access to the spreadsheet. Rahmadi plz verify.}

\myparagraph{Time Window and Signature Duration.}
We also measured the duration of our signatures---defined as the time
 between the first and the last packets of the signature.
The results are summarized in
Tables~\ref{tab:wan-signatures} and \ref{tab:lan-signatures}.
The longest signature duration is 8,431 ms (less than 9 sec) for
the \blossomsprinkler's ON event from the device's communication.
This justifies our choice of time window \timewindow = 15 seconds
during trace filtering and signature validation 
(see Sec.~\ref{sect:system-training}).  This conservative  choice 
also provides slack to accommodate other devices that we have not evaluated and might have 
signatures with a longer duration.

\myparagraph{Matching.}
For detection, we use strict time constraints.
A signature match is declared when all matching packet sequence sets occur within 
the duration $\lceil t + 0.1t \rceil$ with $t$ being the maximum observed signature 
duration (see Tables~\ref{tab:wan-signatures} and~\ref{tab:lan-signatures}).

% While we currently use the same 15-second time constraint during detection,
% we point out that one could use this knowledge of signature duration to make
% detection more temporally strict and thereby potentially reduce the false positive rate. 
% \todo{Remove if we actually rerun with stricter time constraints.}

%DBSCAN needs to be configured with the right values for its parameters, 
%namely $\epsilon$ and $\mathtt{minPts}$.
%Our DBSCAN clusterer attempts to scan all the pairs while forming clusters---a
%cluster consists of \emph{core} and \emph{non-core} pairs. 
%A pair is labeled as a core pair in the cluster if at least $\mathtt{minPts}$ pairs are within 
%the distance $\epsilon$ (\ie maximum radius of a core pair's neighborhood).
%When a pair is reachable from a core pair but have less than $\mathtt{minPts}$ 
%neighboring pairs within $\epsilon$, it becomes a non-core pair.
%If a pair is not reachable from any of the core pairs in a forming cluster,
%it is labeled as noise.

%Since we want to generate a unique signature for every device, we have to
%harvest the tightest clusters available among all pairs.
%First, we need to pick a $\mathtt{minPts}$ value that is closest to the size
%that we desire for our clusters.
%Hence, $\mathtt{minPts}$ has to be close to the number of events---a pair 
%is desired if it appears coincidentally with one event.
%We assign $\mathtt{minPts}=\lfloor n-0.1n \rfloor$, where $n$ is the total 
%number of events.
%The slack of $0.1n$ is given to $\mathtt{minPts}$ to take into account that 
%event-related traffic could occasionally have missing pairs caused by
%the phone app not being responsive for some of the triggers or the pairs
%may have variations that cannot be captured in the pair clustering,
%\eg \code{S-777 C-136} for the Samsung SmartThings plug may occassionally 
%vary into \code{S-612 C-136}.
%%\todo{How is this possible if we collect data at the router?  What really happens}
%Second, we need to pick the smallest $\epsilon$ value possible to ensure
%that the formed cluster is tight. For this purpose, we conservatively
%picked $\epsilon=10$. This is to accommodate devices that may have slight
%variations in the pairs. 
%For instance, our further observation shows that 
%the D-Link plug's packet pair of lengths 1117 and 613 that represent a ``toggle ON''
%(see Sec.~\ref{sect:observation}) event event can have variation in the first packet 
%length---it can be any odd number between 1109 and 1123.

\subsection{Smart Home Testbed Experiment}
\label{sect:detection-phase}
\myparagraph{Testing Dataset.}
To see how effective the packet-level signatures are in detecting \events,
we collected network traces and used \tool to perform detection 
on them.
We used the setup for dataset collection presented in 
Sec.~\ref{sect:experimental-testbed} to collect one dataset for every device.
While collecting a dataset, we generated \events for the device under test. 
At the same time, we also connected the other 12 devices and activated
them (\eg toggled the smart plugs ON) so that they would generate network
traffic. However, we do not generate \events for these other devices.

To generate Background Traffic as depicted in Fig.~\ref{fig:combined-setup},
we also set up 3 general purpose devices: a Motorola moto g$^6$ phone that would play
a Youtube video playlist, a Google Nexus 5 phone that would play a
Spotify song playlist, and an Apple MacBook Air that would randomly
browse top 10 websites~\cite{topwebsites} every 10-500 seconds.
With this setup, we tried to emulate the network traffic from a smart
home when all devices are active.

\myparagraph{Results Summary.}
Despite our strict matching strategy of requiring
exact matches 
to the actual instances of packet sequences in the detection dataset, 
the average accuracy of our 
packet-level signatures is 97.4\%---ranging between 92-100 matches
per 100 expected events---for the 12 devices with
signatures (see Tables~\ref{tab:wan-signatures-accuracy} 
and~\ref{tab:lan-signatures}).
%\todo{Do we want to be clear that we did not actually do Wi-Fi sniffing
%for packet collection?}
The results are the same for both WAN sniffer and Wi-Fi sniffer matching strategies.

\myparagraph{False Positives.}
For both strategies, we have a low rate of true false positives. Overall,
there are only 2 true false positives for both strategies for the \arlocamera, and 
3 true false positives for the Wi-Fi sniffer matching of the \nestthermostat.

\mysubparagraph{\dlinkplug.}
\tool detected 95/100 events for the \devicecloudcomm signature. 
Manual inspection revealed that 5 events were not detected because the signature only appeared partially in those events.
For the \phonecloudcomm signatures, \tool detected 98/100 events. 
Manual inspection revealed that the 2 undetected events exhibit sequences
%(\ie \code{<C-1125, S-613>} and \code{<C-1126, S-613>}) 
that have not been covered by the signatures.
%---we recommend bigger training sets.
%Therefore, we recommend collecting bigger network traces with more events 
%as training sets to provide better signature coverage.

\mysubparagraph{\tplinkplug.}
\tool detected 99/100 events for the \devicecloudcomm signatures.
Manual inspection confirmed that 1 event was not detected because the event exhibited a sequence that was not covered by the signature.
For the Wi-Fi sniffer matching, we combined both 
\devicecloudcomm and \phonedevicecomm signatures
since both are observable in this adversary model.
%(\ie \code{<556, 1294>}).

\mysubparagraph{\dlinksiren and \kwiksetdoorlock.}
\tool successfully detected all 100 events for both devices.
The Wi-Fi sniffer matching only yielded 2 false positives
for the OFF-event signature among 694,045 packets in the captured trace.
However, both of them were caused by signature packet retransmissions, thus both are not true false positives.

\mysubparagraph{\smartthingsplug.}
\tool detected 92/100 events for the \phonecloudcomm signatures.
Manual inspection revealed that 8 events were not detected because the signatures were only partially present, or had other variations that were not covered by the generated signature, during those events.

\mysubparagraph{\arlocamera.}
\tool initially detected only 55/100 events for the \phonecloudcomm signatures.
Manual inspection revealed that there were a lot of variations for set \code{S2} in the ON signature that were not covered during training.
For instance, while the training set covered \code{C-271 S-503} and \code{C-272 S-503}, it did not cover \code{C-273 S-503}.%---hence, coverage problem.
%\todo{I am not sure if there is a better way to position this?}
When we used only the set \code{S1} for ON-event detection, \tool detected 97/100 events.
The WAN and Wi-Fi sniffer matching strategies both yielded 2 
false positives for the OFF-event signature among 1,957,724 packets in the captured trace. 
%These 2 false positives were detected in the camera initialization phase.

\mysubparagraph{\nestthermostat.}
\tool detected 93/100 events for the \phonecloudcomm signatures. Seven events were
missing also because of variations that have not been covered by the signatures.
The Wi-Fi sniffer matching yielded 8 false positives, 5 for
OFF-event signature and 3 for ON-event signature from 696,941 packets in 
the captured trace. However, further investigation revealed that 5 false positives
were caused by retransmissions---only 3 are true false positives.
%\todo{double check this!}
%For 2 of these 3 true false positives, the durations between the first and the last
%packets are way longer than the maximum duration (\ie 1,072 ms) of the actual 
%signatures (see Table~\ref{tab:wan-signatures}). Thus applying a stricter detection
%time constraint reduced the number of false positives down to 1
%(see Sec.~\ref{sect:parameter-sensitivity}).

%\subsubsection{LAN Signatures}
\myparagraph{\phonedevicecomm Signatures.}
We use the Wi-Fi sniffer matching strategy for the devices that exhibit
signatures in the \phonedevicecomm communication.
\tool detected all 100 events for every device 
(see Table~\ref{tab:lan-signatures}).
Although each signature consists of only 2-3 packets in 1 set of packet 
sequences, none of the signatures generated false positives.

%We could not run the detection experiment for the Philips Hue White because 
%some firmware change made the previously detected signatures disappeared.

%\begin{table}[t!]
%  \centering
%  \begin{center}
%  { \footnotesize
%  \begin{tabular}{| l | r | r | r |}
%    \hline
%        No. & File & Size & \# Packets\\
%    \hline
%        1 & 16-09-23.pcap & 370MB & 947,072\\
%    \hline
%        2 & 16-09-24.pcap & 338.7MB  & 799,235\\
%    \hline
%        3 & 16-09-25.pcap & 102.2MB & 537,650\\
%    \hline
%        4 & 16-09-26.pcap & 114.4MB & 573,848\\
%    \hline
%        5 & 16-09-27.pcap & 89.6MB & 527,035\\
%    \hline
%        6 & 16-09-28.pcap & 1.2GB & 2,019,000\\
%    \hline
%        7 & 16-09-29.pcap & 156.1MB & 738,906\\
%    \hline
%        8 & 16-10-01.pcap & 145.3MB & 736,136\\
%    \hline
%        9 & 16-10-02.pcap & 105.3MB & 607,202\\
%    \hline
%        10 & 16-10-03.pcap & 119.0MB & 670,160\\
%    \hline
%        11 & 16-10-04.pcap & 2.2GB & 2,344,991\\
%    \hline
%        12 & 16-10-05.pcap & 653.0MB & 1,655,879\\
%    \hline
%        13 & 16-10-06.pcap & 171.4MB & 719,243\\
%    \hline
%        14 & 16-10-07.pcap & 685.9MB & 1,362,858\\
%    \hline
%        15 & 16-10-08.pcap & 114.6MB & 612,210\\
%    \hline
%        16 & 16-10-09.pcap & 101.4MB & 559,444\\
%    \hline
%        17 & 16-10-10.pcap & 104.3MB & 580,488\\
%    \hline
%        18 & 16-10-11.pcap & 1.2GB & 2,073,339\\
%    \hline
%        19 & 16-10-12.pcap & 4.5GB & 4,948,806\\
%    \hline
%    \hline
%    	& Total & 12.5GB & 23,013,502\\
%    \hline
%  \end{tabular}
%  }
%  \end{center}
%  \caption{PCAP files for negative control experiment from~\cite{sivanathan-classifier}.
%  	\label{tab:pcap-files}}
%\end{table}

% \begin{table}[t!]
  % \centering
  % \begin{center}
  % { \footnotesize
  % \begin{tabular}{| l | r | r |}
  	% \hline
  		% \textbf{Device} & \multicolumn{2}{| c |}{\textbf{Phone-Cloud}}\\
         % & \multicolumn{2}{| c |}{\textbf{Signature}} \\
    % \cline{2-3}
    	 % & \textbf{ON} & \textbf{OFF}\\
    % \hline
        % \dlinkplug & 11 & 6\\
    % \hline
        % \dlinksiren & 2 & 1\\
    % \hline
        % \arlocamera & 0 & 1\\
    % \hline
        % \nestthermostat & 8 & 4\\
    % \hline
        % \blossomsprinkler & 0 & 1\\
    % \hline
        % \huebulb & 1 & 3\\
    % \hline
  % \end{tabular}
  % }
  % \end{center}
  % \caption{False positives of Wi-Fi sniffer matching on negative 
  	% dataset 2 (simulated office-space traffic dataset).
  	% \label{tab:false-positives}}
% \end{table}

\subsection{Negative Control Experiment}
\label{sect:negative-control}%
%\todo{Could use better explanation...The traffic presumably does not include devices in 
%question and thus we should expect to see 0 signature matches??}
If the packet-level signatures are to be used to detect events in a real 
setting, they must be sufficiently unique for each device 
compared to other traffic to avoid generating false positives. 
We evaluated the uniqueness of the signatures by performing signature 
detection on two datasets. 
%\todo{Not exactly true: I only tested the WAN signatures for CICIDS2017}
The first dataset consists of traffic generated by similar devices (\ie other smart 
home devices), while the second dataset serves to evaluate the uniqueness 
of the signatures among traffic generated by general purpose computational devices.
%\todo{Need to update this part. Probably need to create a table!}

\myparagraph{Negative Dataset 1: UNSW Smart Home Traffic Dataset.}
The first dataset ~\cite{sivanathan-classifier} contains network traces for 
26 smart home devices that are \emph{different} from the devices that 
we generated signatures for. 
%\footnote{The dataset \emph{does} 
%contain data for Belkin WeMo and the TP-Link HS-110, which are also in our 
%set of devices. However, in~\cite{sivanathan-classifier}, these devices 
%communicate using TLSv1.0 while they communicate using TLSv1.2 in our 
%traces. We suspected that this is to be attributed to older firmware versions, 
%and that this is the reason why we did not see any matched signatures for 
%these two devices.}. 
The list of devices can be found in~\cite{devicelist}. 
The dataset is a collection of 19 PCAP files, with a total size of 12.5GB and a total packet 
count of 23,013,502.
%\footnote{The full dataset 
%actually consists of 20 PCAP files, but one PCAP file could not be downloaded 
%due to permission issues.}
%(see Table~\ref{tab:pcap-files})
%\todo{Table doesn't 
%really add any value, consider dropping it.}

\myparagraph{Negative Dataset 2: UNB Simulated Office-Space Traffic Dataset.}
This is the Monday trace of the CICIDS2017 
dataset~\cite{sharafaldin2018toward} and it contains simulated network traffic 
for an office space with two servers and 10 laptops/desktops with diverse 
operating systems.
The dataset we used is a single PCAP file of 10.82GB, with a total of 11,709,971 
packets observed at the WAN interface.
%\footnote{The full trace contains 11,709,971 packets, but we filtered 
%the trace, dropping all non-IP traffic and traffic between two local machines, 
%as we were interested in evaluating the uniqueness of WAN signatures.}. 
%\todo{Small issue with these numbers as I filtered the trace to only contain 
%WAN traffic...}

\myparagraph{Results Summary.}
For both datasets, we performed signature detection for all devices
using the WAN sniffer strategy for devices with \phonecloudcomm and 
\devicecloudcomm signatures, and the 
Wi-Fi sniffer strategy for all 12 devices.
For the WAN sniffer, there was no false positive 
across 23,013,502 packets in negative dataset 1, while there is 1 false positive for the
\nestthermostat across 11,709,971 packets in negative dataset 2.
For the Wi-Fi sniffer, \tool detected some false positives due to its
more relaxed matching strategy (see Sec.~\ref{sect:system-detection}).
For the negative dataset 1, \tool detected 
1 false positive for the \dlinkplug,
1 false positive for the \blossomsprinkler,
2 false positives for the \arlocamera, 
2 false positives for the \huebulb, and
4 false positives for the \nestthermostat, each across 23,013,502 packets.
For the negative dataset 2, \tool detected 
1 false positive for the \arlocamera,
1 false positive for the \blossomsprinkler, 
2 false positives for the \dlinksiren, 
4 false positives for the \huebulb,
12 false positives for the \nestthermostat, and 
17 false positives for the \dlinkplug, each across 11,709,971 packets.

All the false positives were detected for signatures that consist of
only 1 pair of packets---longer signatures
did not generate any false positives.
More false positives were detected from the negative dataset 2 presumably because 
this dataset contains traffic from general purpose computing
devices---hence, more traffic variety.
These results show that
the extracted packet-level signatures are unique: the average is 2 false positives
per device for the negative dataset 1 across 23,013,502 packets and 3 false positives 
per device for the negative dataset 2 across 11,709,971 packets.
%---without
%any additional information such as IP addresses or hostnames of the endpoints.

%This dataset aids in investigating the uniqueness of the detected signatures 




==> overview.tex <==
%\section{Overview}
\section{General Case and Problem Statement}
\label{sect:overview}
\subsection{Objectives}
\label{sect:motivation}
The case study described in Sec.~\ref{sect:network-behavior} suggests
that packet-level analysis can infer the types of events from smart
plugs' encrypted network traffic.  Motivated by the results from our
case study, we next develop an automatic approach to inferring and
checking for signatures.  We have developed a system that can (1)
automatically collect data and perform packet-level analysis to
extract packet-level signatures, and (2) use the generated
packet-level signature to detecting IoT events by monitoring a network
trace.

Furthermore, once we started inspecting more devices and collected more data, 
it became clear that some devices would in fact exhibit deterministic 
behavior in their packet exchanges although with slight variations. 
For example, we observed that the length 
of the first packet sent by the phone when the D-Link smart plug was toggled ON or OFF
would vary slightly around the initially reported values in such a way that all ON
events would result in an odd number (\eg 1115, 1117, 1119, etc.), 
whereas all OFF events would result in an even number (\eg 1116, 1118, 
1120, etc.).


\subsection{Research Questions}
\label{sect:design}

There are three research questions that must be answered
While designing our approach, we asked the following 3 research questions 
as our guidelines.

\myparagraph{RQ1: How do we automate the collection of the network traffic that 
serves as input to the packet-level analysis?}
Basically, we need a means to automatically trigger the smartphone app
of a smart home device to generate certain types of events on the device.

\myparagraph{RQ2: How do we automatically extract packet-level signatures from 
the collected data?}
Sec.~\ref{sect:observation} has presented the format of packet-level signatures in the form of 
sequences of packets that consist of pairs of \emph{request-reply} communication packets
between a device and an endpoint (\eg an Internet host).
The system must first discern event-related traffic (\ie
traffic that occurs immediately after a user action, \eg toggle ON)
from unrelated traffic, and subsequently examine the event-related traffic to find recurring
patterns. While the first step is clearly a filtering problem, the
second step is less obvious due to the slight variations in the
packet lengths (see Sec.~\ref{sect:motivation}) 
coupled with the unbounded complexity of packet-level 
signatures---single packet pairs for the D-Link plug vs. multiple packet pairs in 2 different
TCP connections for the SmartThings plug (see Table~\ref{tab:packet-level-signatures}).

%a signature 
%may be as simple as a single packet pair occurring on a single TCP connection
%(\eg the D-Link plug in Table~\ref{tab:packet-level-signatures}),
%or as complex as multiple, long packet sequences occurring on
%different TCP connections (\eg the SmartThings Outlet in 
%Table~\ref{tab:packet-level-signatures}).

\myparagraph{RQ3: How do we detect the occurrence of
a packet-level signature in a network trace?}
Since signatures can be comprised of multiple packet sequences
occurring on different TCP connections, but within close
temporal proximity of one another, we need an algorithm that first matches
the individual packet sequences, and then enforces the inter-sequence
temporal relationship. 
%Furthermore, to enable a real-time 
%version of the attack described in Sec.~\ref{sect:threat-model}, this
%algorithm should be efficient and effective---\emph{not} a brute-force search.

\todo{The adversary model needs to wait for the attack model discussion}
\todo{Do we want to talk about the C-S notation here?}
\input{threat-model}


